Defeasible RDFS via Rational Closure

In the field of non-monotonic logics, the notion of Rational Closure (RC) is acknowledged as a prominent approach. In recent years, RC has gained even more popularity in the context of Description Logics (DLs), the logic underpinning the semantic web standard ontology language OWL 2, whose main ingredients are classes and roles. In this work, we show how to integrate RC within the triple language RDFS, which together with OWL2 are the two major standard semantic web ontology languages. To do so, we start from $\rho df$, which is the logic behind RDFS, and then extend it to $\rho df_\bot$, allowing to state that two entities are incompatible. Eventually, we propose defeasible $\rho df_\bot$ via a typical RC construction. The main features of our approach are: (i) unlike most other approaches that add an extra non-monotone rule layer on top of monotone RDFS, defeasible $\rho df_\bot$ remains syntactically a triple language and is a simple extension of $\rho df_\bot$ by introducing some new predicate symbols with specific semantics. In particular, any RDFS reasoner/store may handle them as ordinary terms if it does not want to take account for the extra semantics of the new predicate symbols; (ii) the defeasible $\rho df_\bot$ entailment decision procedure is build on top of the $\rho df_\bot$ entailment decision procedure, which in turn is an extension of the one for $\rho df$ via some additional inference rules favouring an potential implementation; and (iii) defeasible $\rho df_\bot$ entailment can be decided in polynomial time.

==> common.tex <==
\usepackage{times,url,graphicx,latexsym,xspace,%
eurosym,amssymb,amsmath,helvet,courier}

\usepackage[ruled]{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{amsthm}

%\usepackage[ruled,vlined]{algorithm2e}

%\usepackage{algorithm}
%\usepackage{algorithmic}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}
%\renewcommand{\mathtt}[1]{\mathit{#1}}
\renewcommand{\P}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\AU}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\AP}{\ensuremath{\mathbf{P}}\xspace}
\newcommand{\AB}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\AL}{\ensuremath{\mathbf{L}}\xspace}
\newcommand{\AV}{\ensuremath{\mathbf{V}}\xspace}
\newcommand{\AUBL}{\ensuremath{\mathbf{UBL}}\xspace}
\newcommand{\AUB}{\ensuremath{\mathbf{UB}}\xspace}
\newcommand{\AUL}{\ensuremath{\mathbf{UL}}\xspace}
\renewcommand{\AA}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\AULV}{\ensuremath{\mathbf{ULV}}\xspace}
\newcommand{\AUV}{\ensuremath{\mathbf{UV}}\xspace}


\renewcommand{\O}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\A}{\ensuremath{\mathcal{A}}\xspace}
\renewcommand{\k}{\ensuremath{k}\xspace}
\renewcommand{\a}{\ensuremath{a}\xspace}

\newcommand{\sub}{\ensuremath{\sqsubseteq}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\K}{\ensuremath{\mathcal{K}}\xspace} 
\newcommand{\T}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\F}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\I}{\ensuremath{\mathcal{I}}\xspace}      
\newcommand{\J}{\ensuremath{\mathcal{J}}\xspace}   
\newcommand{\IA}{\ensuremath{\mathcal{I}_{\A}}\xspace}      
\newcommand{\R}{\ensuremath{\mathcal{R}}}
\newcommand{\m}{\I\xspace}
\newcommand{\f}{\ensuremath{f}\xspace}
\newcommand{\s}{\ensuremath{s}\xspace}
\newcommand{\x}{\ensuremath{x}\xspace}
\newcommand{\nd}{\noindent}
\newcommand{\calK}{{\cal K}}
\newcommand{\calF}{{\mathcal F}}
\newcommand{\calL}{{\mathcal L}}
\newcommand{\calS}{{\mathcal S}}
\newcommand{\lpx}[1]{{\mathcal #1}}
\newcommand{\lp}{\lpx{P}}
\newcommand{\ground}[1]{\mathtt{ground}(#1)}
\newcommand{\tuple}[1]{\langle #1 \rangle }
\newcommand{\triple}[1]{(#1)}
\newcommand{\entail}{\models}
\newcommand{\unitn}{[0,1]_{m}}
\newcommand{\andc}{\sqcap}
\newcommand{\all}{\forall}
\newcommand{\some}{\exists}
\newcommand{\somei}[2]{\some #1\colon \!\! #2}
\newcommand{\notc}{\neg}
\newcommand{\orc}{\sqcup}
\newcommand{\csome}{\exists}
\newcommand{\atleast}[1]{\geq #1\ }
\newcommand{\atmost}[1]{\leq #1\ }
\newcommand{\bottomc}{\perp}
\newcommand{\topc}{\top}
\newcommand{\impc}{\sqsubseteq}
\newcommand{\highi}[1]{{#1}^{\cal I} }
\newcommand{\term}[1]{\ensuremath{\mbox{\small$\mathtt{#1}$}}}
%\newcommand{\uri}[1]{\ensuremath{\term{{:}#1}}}
\newcommand{\uri}[1]{\ensuremath{\term{#1}}}
\newcommand{\bnode}[1]{\ensuremath{\term{{\mathunderscore:}#1}}}


\newcommand{\eval}[1]{[\![ #1 ]\!]}


%\newcommand{\assign}{\colon\!\!\!\!=}
\newcommand{\assign}{\mbox{$\colon\!\!\!\!=$}}

\newcommand{\fg}[1]{\tilde{#1}}

%\newcommand{\intP}[1]{{#1}^{\I_{P}} }
%\newcommand{\intC}[1]{{#1}^{\I_{C}} }
\newcommand{\intL}[1]{{#1}^{\I_{L}} }
\newcommand{\intA}[1]{{#1}^{\I_{\A}} }
%\newcommand{\intGA}[1]{{#1}^{{\I_G}_{\A}} }
\renewcommand{\int}[1]{{#1}^{\I} }
\newcommand{\intG}[1]{{#1}^{\I_G} }
\newcommand{\intGs}[1]{{#1}^{\I_{G^s}} }
\newcommand{\intGA}[1]{{#1}^{\I_{G,A}} }
%\newcommand{\intP}[1]{{[\![#1]\!]}_{P}}
\newcommand{\intP}[1]{{\mathfrak{P}[\![#1]\!]}}
%\newcommand{\intC}[1]{{[\![#1]\!]}_{C}}
\newcommand{\intC}[1]{{\mathfrak{C}[\![#1]\!]}}

\newcommand{\spp}{\ensuremath{\mathsf{sp}}}
\newcommand{\subclass}{\ensuremath{\mathsf{sc}}}
\newcommand{\type}{\ensuremath{\mathsf{type}}}
\newcommand{\dom}{\ensuremath{\mathsf{dom}}}
\newcommand{\range}{\ensuremath{\mathsf{range}}}
\newcommand{\eee}{\ensuremath{\mathsf{e}}}

\newcommand{\ii}[1]{\mbox{$(#1)$}}

%\newcommand{\fuzzyg}[2]{\mbox{$\langle #1, #2\rangle$}}
%\newcommand{\fuzzyg}[2]{\mbox{$#1[#2]$}}
\newcommand{\fuzzyg}[2]{\mbox{$#1\colon#2$}}

\newcommand{\FKB}{{\lp}}
\newcommand{\maps}{\mapsto}

\newcommand{\aggr}{@}
\newcommand{\comp}{\circ}


\newcommand{\dldb}{{\subclass DL-DB}}
%\newtheorem{example}{Example}
%\newtheorem{proposition}{Proposition}
\newcommand{\okex}{ \hfill $\Box$}
%\renewcommand{\vec}{\mathbf}
\renewcommand{\vec}[1]{\bar{\mathbf #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros

 \newtheorem{theorem}{Theorem}[section]
 \newtheorem{proposition}[theorem]{Proposition}
 \newtheorem{corollary}[theorem]{Corollary}
 \newtheorem{lemma}[theorem]{Lemma}

 \newtheorem{example}{Example}[section]
 \newtheorem{definition}{Definition}[section]
% \newtheorem{proof}{Proof}[section]
\newtheorem{remark}{Remark}[section]

%\newcommand{\qed}[0]{\hspace*{1em}\hbox{\proofbox}}

% \newtheorem{zdefinition}{Definition}[section]
% \newenvironment{definition}[1][\mbox{}]{\begin{zdefinition}\begin{rm}#1}{\end{rm}\end{zdefinition}}

% \newtheorem{zexample}{Example}[section]
% \newenvironment{example}[1][\mbox{}]{\begin{zexample}\begin{rm}#1}{\end{rm}\end{zexample}}


 %% No numbered paragraphs
 \setcounter{secnumdepth}{3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\spec}{{\mbox{$\tau$}}}
\newcommand{\astat}{{\mbox{$\sigma$}}}

\newcommand{\ie}{\textit{i.e.},\xspace}
\newcommand{\eg}{\textit{e.g.},\xspace}
\newcommand{\viz}{\textit{viz.},\xspace}
\newcommand{\wrt}{w.r.t.\xspace}
\newcommand{\D}{{\mathtt D}}
\newcommand{\etal}{\textit{et al.}\xspace}
\renewcommand{\iff}{if and only if\xspace}
\newcommand{\st}{such that\xspace}


\newcommand{\rhodf}{\mbox{$\rho$df}\xspace}
\newcommand{\universe}{\ensuremath{\mathtt{uni}}\xspace}
\newcommand{\voc}{\ensuremath{\mathtt{voc}}\xspace}

%\newcommand{\algorithm}[1]{
%\begin{center}
%\fbox{
%\begin{minipage}{0.96\textwidth}
%\footnotesize\smallskip

%#1

%\end{minipage}
%}
%\end{center}
%}



\newcommand{\ges}{\,{\geqslant}\,}
\newcommand{\les}{\,{\leqslant}\,}
\newcommand{\ins}{\,{\in}\,}
\newcommand{\notf}{\neg}
\newcommand{\orf}{\lor}
\newcommand{\andf}{\land}
\newcommand{\impf}{\rightarrow}
\newcommand{\unit}{[0,1]}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\KB}{\mathit{K\!B}}
\newcommand{\eqs}{\,{=}\,}
\newcommand{\mids}{\,{\mid}\,}

\newcommand{\notr}{\neg}


\newcommand{\stt}[1]{\texttt{{\small#1}}}


%\newtheorem{example}{Example}
%\newtheorem{proposition}{Proposition}


\def\qed{\hspace*{\fill} \ensuremath{\Box}}

% \comment{extending the SPARQL algebra, copy of Axel's sparqlog}
\def\NULL{{\sf null}\xspace}
\newcommand{\louter}{{\sqsupset\!\!\!}\bowtie}
\newcommand{\lms}{\ensuremath{\{\!\!\{}}
\newcommand{\rms}{\ensuremath{\}\!\!\}}}
\newcommand{\Tnull}{\ensuremath{T_\NULL}}
\newcommand{\blank}[1]{\ensuremath{\_\!\_\!{:}\!\mathtt{#1}}}


% \newcommand{\aSPARQL}{SPRINQL\xspace}
%\newcommand{\aSPARQL}{annotated SPARQL\xspace}
\newcommand{\aSPARQL}{AnQL\xspace}

% \newcommand{\tinyotimes}{\mbox{\tiny $\otimes$}}
\newcommand{\cupotimes}{\ensuremath{\ \mathaccent\cdot\cup \ }}

%commands for the Big oplus and Big otimes, to get the indices that Axel wants ;)
\newcommand{\bigoplusone}[1]{{{\bigoplus_1}\atop{\text{\tiny$#1$}}}}
\newcommand{\bigoplustwo}[1]{{{\bigoplus_2}\atop{\text{\tiny$#1$}}}}
\newcommand{\bigotimesone}[1]{{{\bigotimes_1}\atop{\text{\tiny$#1$}}}}
\newcommand{\bigotimestwo}[1]{{{\bigotimes_2}\atop{\text{\tiny$#1$}}}}
%commands for the Big oplus and Big otimes without the indices
%\newcommand{\bigoplusone}[1]{\bigoplus_{#1}}
%\newcommand{\bigoplustwo}[1]{\bigoplus_{#1}}
%\newcommand{\bigotimesone}[1]{\bigotimes_{#1}}
%\newcommand{\bigotimestwo}[1]{\bigotimes_{#1}}

\newcommand{\bigorone}[1]{{{\bigor_1}\atop{\text{\tiny$#1$}}}}
\newcommand{\bigortwo}[1]{{{\bigor_2}\atop{\text{\tiny$#1$}}}}
\newcommand{\bigandone}[1]{{{\bigand_1}\atop{\text{\tiny$#1$}}}}
\newcommand{\bigandtwo}[1]{{{\bigand_2}\atop{\text{\tiny$#1$}}}}








\newcommand{\intLabel}[1]{\pgfmathparse{2000+#1} \pgfmathtruncatemacro{\res}{\pgfmathresult} \res}

\newcommand{\makegraph}[2]{
  \begin{tikzpicture}[scale=0.65]
    \tikzstyle{every node}=[gray,font=\scriptsize]
    \draw (0,0) node[left]{$T_1$} -- (10,0) ;
    \foreach \startPoint/\endPoint in #1
    {
      \draw[line width=2mm] (\startPoint,0) node[above]{\intLabel{\startPoint}} -- (\endPoint,0) node[above]{\intLabel{\endPoint}};
    }

    \draw (0,-1) node[left]{$T_2$} -- (10,-1) ;
    \foreach \startPoint/\endPoint in #2
    {
      \draw[line width=2mm] (\startPoint,-1) node[below]{\intLabel{\startPoint}} -- (\endPoint,-1) node[below]{\intLabel{\endPoint}};
    }

  \end{tikzpicture}
}

%%% Local Variables:
%%% mode: latex
%%% mode: flyspell
%%% mode: reftex
%%% TeX-master: "DERI-TR-annotatedRDF"
%%% End:




